Multiscale and Nonlocal Learning for PDEs using Densely Connected RNNs

Learning time-dependent partial differential equations (PDEs) that govern evolutionary observations is one of the core challenges for data-driven inference in many fields. In this work, we propose to capture the essential dynamics of numerically challenging PDEs arising in multiscale modeling and simulation -- kinetic equations. These equations are usually nonlocal and contain scales/parameters that vary by several orders of magnitude. We introduce an efficient framework, Densely Connected Recurrent Neural Networks (DC-RNNs), by incorporating a multiscale ansatz and high-order implicit-explicit (IMEX) schemes into RNN structure design to identify analytic representations of multiscale and nonlocal PDEs from discrete-time observations generated from heterogeneous experiments. If present in the observed data, our DC-RNN can capture transport operators, nonlocal projection or collision operators, macroscopic diffusion limit, and other dynamics. We provide numerical results to demonstrate the advantage of our proposed framework and compare it with existing methods.

==> Dense RNN for Multiscale and Nonlocal Learning/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Multiscale and Nonlocal Learning for PDEs}{D. Ricardo, H. Jingwei, and Y. Haizhao}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Multiscale and Nonlocal Learning for PDEs using Densely Connected RNNs\thanks{Submitted to the editors DATE.
\funding{RD was partially supported by the Fog Research Institute under contract no.~FRI-454.  JH was partially supported by NSF CAREER grant DMS-1654152. HY was partially supported by NSF CAREER grant DMS-1945029.
}}}

% Authors: full names plus addresses.
\author{Ricardo A. Delgadillo\thanks{Department of Civil and Environmental Engineering, National University of Singapore, Singapore (\email{ceerad@nus.edu.sg}).}
%\thanks{Imagination Corp., Chicago, IL 
 % (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Jingwei Hu\thanks{Department of Mathematics, Purdue University, West Lafayette, IN 47907, USA (\email{jingweihu@purdue.edu}).}
\and Haizhao Yang\thanks{Department of Mathematics, Purdue University, West Lafayette, IN 47907, USA (\email{haizhao@purdue.edu}).}}

%\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

